PatchIsland: Orchestration of LLM Agents for Continuous Vulnerability Repair

Continuous fuzzing platforms such as OSS-Fuzz uncover large numbers of vulnerabilities, yet the subsequent repair process remains largely manual. Unfortunately, existing Automated Vulnerability Repair (AVR) techniques -- including recent LLM-based systems -- are not directly applicable to continuous fuzzing. This is because these systems are designed and evaluated on a static, single-run benchmark setting, making them ill-suited for the diverse, noisy, and failure-prone environments in continuous fuzzing. To address these issues, we introduce PatchIsland, a system for Continuous Vulnerability Repair (CVR) that tightly integrates with continuous fuzzing pipelines. PatchIsland employs an ensemble of diverse LLM agents. By leveraging multiple LLM agents, PatchIsland can cover a wider range of settings (e.g., different projects, bug types, and programming languages) and also improve operational robustness. In addition, PatchIsland utilizes a two-phase patch-based deduplication to mitigate duplicate crashes and patches, which can be problematic in continuous fuzzing. In our internal evaluation, PatchIsland repaired 84 of 92 vulnerabilities, demonstrating strong repair capability. In the official AIxCC competition, the system operated with no human intervention in a fully autonomous environment and successfully patched 31 out of 43 vulnerabilities, achieving a repair rate of 72.1\%.

==> code/fmt.tex <==

\makeatletter
\def\PY@reset{\let\PY@it=\relax \let\PY@bf=\relax%
    \let\PY@ul=\relax \let\PY@tc=\relax%
    \let\PY@bc=\relax \let\PY@ff=\relax}
\def\PY@tok#1{\csname PY@tok@#1\endcsname}
\def\PY@toks#1+{\ifx\relax#1\empty\else%
    \PY@tok{#1}\expandafter\PY@toks\fi}
\def\PY@do#1{\PY@bc{\PY@tc{\PY@ul{%
    \PY@it{\PY@bf{\PY@ff{#1}}}}}}}
\def\PY#1#2{\PY@reset\PY@toks#1+\relax+\PY@do{#2}}

\@namedef{PY@tok@w}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\@namedef{PY@tok@c}{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.24,0.48,0.48}{##1}}}
\@namedef{PY@tok@cp}{\def\PY@tc##1{\textcolor[rgb]{0.61,0.40,0.00}{##1}}}
\@namedef{PY@tok@k}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@kp}{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@kt}{\def\PY@tc##1{\textcolor[rgb]{0.69,0.00,0.25}{##1}}}
\@namedef{PY@tok@o}{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PY@tok@ow}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\@namedef{PY@tok@nb}{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@nf}{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\@namedef{PY@tok@nc}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\@namedef{PY@tok@nn}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\@namedef{PY@tok@ne}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.80,0.25,0.22}{##1}}}
\@namedef{PY@tok@nv}{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\@namedef{PY@tok@no}{\def\PY@tc##1{\textcolor[rgb]{0.53,0.00,0.00}{##1}}}
\@namedef{PY@tok@nl}{\def\PY@tc##1{\textcolor[rgb]{0.46,0.46,0.00}{##1}}}
\@namedef{PY@tok@ni}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.44,0.44,0.44}{##1}}}
\@namedef{PY@tok@na}{\def\PY@tc##1{\textcolor[rgb]{0.41,0.47,0.13}{##1}}}
\@namedef{PY@tok@nt}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@nd}{\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\@namedef{PY@tok@s}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@sd}{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@si}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.64,0.35,0.47}{##1}}}
\@namedef{PY@tok@se}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.36,0.12}{##1}}}
\@namedef{PY@tok@sr}{\def\PY@tc##1{\textcolor[rgb]{0.64,0.35,0.47}{##1}}}
\@namedef{PY@tok@ss}{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\@namedef{PY@tok@sx}{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@m}{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PY@tok@gh}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\@namedef{PY@tok@gu}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\@namedef{PY@tok@gd}{\def\PY@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\@namedef{PY@tok@gi}{\def\PY@tc##1{\textcolor[rgb]{0.00,0.52,0.00}{##1}}}
\@namedef{PY@tok@gr}{\def\PY@tc##1{\textcolor[rgb]{0.89,0.00,0.00}{##1}}}
\@namedef{PY@tok@ge}{\let\PY@it=\textit}
\@namedef{PY@tok@gs}{\let\PY@bf=\textbf}
\@namedef{PY@tok@ges}{\let\PY@bf=\textbf\let\PY@it=\textit}
\@namedef{PY@tok@gp}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\@namedef{PY@tok@go}{\def\PY@tc##1{\textcolor[rgb]{0.44,0.44,0.44}{##1}}}
\@namedef{PY@tok@gt}{\def\PY@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\@namedef{PY@tok@err}{\def\PY@bc##1{{\setlength{\fboxsep}{\string -\fboxrule}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}}
\@namedef{PY@tok@kc}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@kd}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@kn}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@kr}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@bp}{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@fm}{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\@namedef{PY@tok@vc}{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\@namedef{PY@tok@vg}{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\@namedef{PY@tok@vi}{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\@namedef{PY@tok@vm}{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\@namedef{PY@tok@sa}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@sb}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@sc}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@dl}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@s2}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@sh}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@s1}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@mb}{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PY@tok@mf}{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PY@tok@mh}{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PY@tok@mi}{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PY@tok@il}{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PY@tok@mo}{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PY@tok@ch}{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.24,0.48,0.48}{##1}}}
\@namedef{PY@tok@cm}{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.24,0.48,0.48}{##1}}}
\@namedef{PY@tok@cpf}{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.24,0.48,0.48}{##1}}}
\@namedef{PY@tok@c1}{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.24,0.48,0.48}{##1}}}
\@namedef{PY@tok@cs}{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.24,0.48,0.48}{##1}}}

\def\PYZbs{\char`\\}
\def\PYZus{\char`\_}
\def\PYZob{\char`\{}
\def\PYZcb{\char`\}}
\def\PYZca{\char`\^}
\def\PYZam{\char`\&}
\def\PYZlt{\char`\<}
\def\PYZgt{\char`\>}
\def\PYZsh{\char`\#}
\def\PYZpc{\char`\%}
\def\PYZdl{\char`\$}
\def\PYZhy{\char`\-}
\def\PYZsq{\char`\'}
\def\PYZdq{\char`\"}
\def\PYZti{\char`\~}
% for compatibility with earlier versions
\def\PYZat{@}
\def\PYZlb{[}
\def\PYZrb{]}
\makeatother



==> fig/agents.tex <==
    \setlength{\fboxsep}{0pt}
    \setlength{\fboxrule}{0.8pt}

    \newlength{\agentboxheight}
    \setlength{\agentboxheight}{3.2cm}

    \begin{minipage}[t]{0.2\linewidth}
        \centering
        \fcolorbox{gray}{white}{%
            \parbox[c][\agentboxheight][c]{\linewidth}{%
                \centering
                \includegraphics[scale=0.8,keepaspectratio=true]{fig/agent/mr.pdf}%
            }%
        }
        \caption*{\parbox{0.9\linewidth}{\centering \sysmr(Single-Agent: Direct Patch)}}
    \end{minipage}%
    \begin{minipage}[t]{0.2\linewidth}
        \centering
        \fcolorbox{gray}{white}{%
            \parbox[c][\agentboxheight][c]{\linewidth}{%
                \centering
                \includegraphics[scale=0.8,keepaspectratio=true]{fig/agent/vincent.pdf}%
            }%
        }
        \caption*{\parbox{0.9\linewidth}{\centering \sysvincent(Single-Agent: Context-Aware Patch)}}
    \end{minipage}%
    \begin{minipage}[t]{0.2\linewidth}
        \centering
        \fcolorbox{gray}{white}{%
            \parbox[c][\agentboxheight][c]{\linewidth}{%
                \centering
                \includegraphics[scale=0.8,keepaspectratio=true]{fig/agent/martian.pdf}%
            }%
        }
        \caption*{\parbox{0.9\linewidth}{\centering \sysmartian (Multi-Agent: Sequential)}}
    \end{minipage}%
    \begin{minipage}[t]{0.2\linewidth}
        \centering
        \fcolorbox{gray}{white}{%
            \parbox[c][\agentboxheight][c]{\linewidth}{%
                \centering
                \includegraphics[scale=0.8,keepaspectratio=true]{fig/agent/claude.pdf}%
            }%
        }
        \caption*{\parbox{0.9\linewidth}{\centering \sysclaudelike (Multi-Agent: Interactive)}}
    \end{minipage}%
    \begin{minipage}[t]{0.2\linewidth}
        \centering
        \fcolorbox{gray}{white}{%
            \parbox[c][\agentboxheight][c]{\linewidth}{%
                \centering
                \includegraphics[scale=0.8,keepaspectratio=true]{fig/agent/prism.pdf}%
            }%
        }
        \caption*{\parbox{0.9\linewidth}{\centering \sysprism (Multi-Agent: Cyclic)}}
    \end{minipage}


==> fig/comparison.tex <==
% Auto-generated by generate_stacked100_per_file.py
% Requires: \usepackage{pgfplots}
% Optional: \usetikzlibrary{patterns}
% Optional grayscale fills replaced by distinct patterns/colors in journal templates
\begin{figure}[htbp]
\centering
\begin{tikzpicture}
\begin{axis}[
  width=0.95\linewidth, height=0.45\linewidth,
  ybar stacked, bar width=12pt,
  ymin=0, ymax=1,
  ytick={0,0.25,0.5,0.75,1.0},
  yticklabels={0\%,25\%,50\%,75\%,100\%},
  xtick=data,
  xticklabel style={rotate=20, anchor=east},
  ylabel={Proportion},
  xlabel={input},
  legend columns=3,
  legend style={at={(0.5,1.02)}, anchor=south, draw=none},
  symbolic x coords={x0,x1,x2,x3,x4},
  xticklabels={buttercup,crete\_parallel,crete\_schedule,crete\_sequential,llm\_analysis}
]
  \addplot+[draw=black, fill=gray!10] coordinates {
    (x0,0.619565) (x1,0.869565) (x2,0.880435) (x3,0.891304) (x4,0.186047)
  };
  \addplot+[draw=black, fill=gray!30, pattern=north east lines] coordinates {
    (x0,0.130435) (x1,0.054348) (x2,0.054348) (x3,0.054348) (x4,0.651163)
  };
  \addplot+[draw=black, fill=gray!50, pattern=north west lines] coordinates {
    (x0,0.163043) (x1,0.076087) (x2,0.065217) (x3,0.054348) (x4,0.000000)
  };
  \addplot+[draw=black, fill=gray!70, pattern=dots] coordinates {
    (x0,0.086957) (x1,0.000000) (x2,0.000000) (x3,0.000000) (x4,0.162791)
  };
  \legend{success, fail, internal_test_failure, error}
\end{axis}
\end{tikzpicture}
\caption{Outcome composition (100\% stacked) from per\_file}
\label{fig:per-file-outcomes-stacked100-pgfplots}
\end{figure}


==> tbl/intended_result_cnt.tex <==
\begin{table*}[h]
    \centering
    \caption{Patch results for intended vulnerabilities. We reproduced each proof-of-vulnerability (PoV) against the corresponding patch using a reference dataset, identifying 99 intended PoVs (including duplicates).}
    \resizebox{0.6\linewidth}{!}{%
        \begin{tabular}{l l r r r}
            \hline
            \textbf{Project Name} & \textbf{Scan Mode} & \textbf{Intended PoV} & \textbf{Patched PoV} & \textbf{Unpatched PoV} \\
            \hline
            commons-compress      & Delta              & 5                     & 5                    & 0                      \\
            curl                  & Delta              & 20                    & 20                   & 0                      \\
            dicoogle              & Full               & 0                     & 0                    & 0                      \\
            freerdp               & Delta              & 1                     & 0                    & 1                      \\
            hdh                   & Full               & 0                     & 0                    & 0                      \\
            hertzbeat             & Full               & 0                     & 0                    & 0                      \\
            jsoup                 & Full               & 0                     & 0                    & 0                      \\
            libexif               & Delta              & 26                    & 26                   & 0                      \\
            libxml2               & Delta              & 10                    & 10                   & 0                      \\
            log4j2                & Delta              & 1                     & 1                    & 0                      \\
            mongoose              & Full               & 1                     & 1                    & 0                      \\
            mongoose              & Delta              & 4                     & 4                    & 0                      \\
            pdfbox                & Full               & 1                     & 1                    & 0                      \\
            pdfbox                & Delta              & 1                     & 0                    & 1                      \\
            shadowsocks           & Full               & 1                     & 1                    & 0                      \\
            systemd               & Full               & 13                    & 0                    & 13                     \\
            tika                  & Delta              & 1                     & 1                    & 0                      \\
            wireshark             & Full               & 7                     & 7                    & 0                      \\
            wireshark             & Delta              & 6                     & 5                    & 1                      \\
            xz                    & Full               & 1                     & 1                    & 0                      \\
            \hline
            \textbf{Total}        &                    & \textbf{99}           & \textbf{83}          & \textbf{16}            \\
            \hline
        \end{tabular}
    }
    \label{tab:intended_result_cnt}
\end{table*}


==> tbl/patch-agent.tex <==
\begin{table}[h]
    \centering
    \caption{Patching agents in \sys (except for open-source agents). Notably, an architecture in this table is just a high-level classification of the agents, and does not imply that the agents are implemented. For that, please refer to the individual agent descriptions.}
    \label{tab:patch-agents-comparison}
    \begin{adjustbox}{max width=\linewidth}
        \begin{tabular}{c C{2.3cm} C{2.5cm} C{4cm}}
            \toprule
            \textbf{Agent} & \textbf{Used models}                          & \textbf{Workflow}                               \\
            \midrule
            \sysmr         & \makecell{Claude 3.7 Sonnet\n OpenAI o4-mini} & \includegraphics[height=0.8cm]{fig/agent/1.pdf} \\
            \midrule
            \sysvincent    & Gemini 2.5 Pro                                & \includegraphics[height=1.0cm]{fig/agent/2.pdf} \\
            \midrule
            \sysmartian    & \makecell{OpenAI o4-mini\n Claude Sonnet 4}   & \includegraphics[height=0.8cm]{fig/agent/3.pdf} \\
            \midrule
            \sysclaudelike & Claude 3.7 Sonnet                             & \includegraphics[height=0.8cm]{fig/agent/4.pdf} \\
            \midrule
            \sysprism      & OpenAI o4-mini                                & \includegraphics[height=0.7cm]{fig/agent/5.pdf} \\
            \bottomrule
        \end{tabular}
    \end{adjustbox}
\end{table}




